Hierarchical MTC User Activity Detection and Channel Estimation with Unknown Spatial Covariance

This paper addresses the joint user identification and channel estimation (JUICE) problem in machine-type communications under the practical spatially correlated channels model with unknown covariance matrices. Furthermore, we consider an MTC network with hierarchical user activity patterns following an event-triggered traffic mode. Therein the users are distributed over clusters with a structured sporadic activity behaviour that exhibits both cluster-level and intra-cluster sparsity patterns. To solve the JUICE problem, we first leverage the concept of strong priors and propose a hierarchical-sparsity-inducing spike-and-slab prior to model the structured sparse activity pattern. Subsequently, we derive a Bayesian inference scheme by coupling the expectation propagation (EP) algorithm with the expectation maximization (EM) framework. Second, we reformulate the JUICE as a maximum a posteriori (MAP) estimation problem and propose a computationally-efficient solution based on the alternating direction method of multipliers (ADMM). More precisely, we relax the strong spike-and-slab prior with a cluster-sparsity-promoting prior based on the long-sum penalty. We then derive an ADMM algorithm that solves the MAP problem through a sequence of closed-form updates. Numerical results highlight the significant performance significant gains obtained by the proposed algorithms, as well as their robustness against various assumptions on the users sparse activity behaviour.

==> commented.tex <==
\begin{comment}
    This section investigate the uses a strong sparsity prior to couple the activity of the UEs amongst each cluster. To this end, we employ a spike and slab function to model the sparsity behaviour of the system. 
 \subsection{The structured spike and slab prior}

In contrast to the majority of the literature on grant-free access MTC that consider random UE activation, we consider herein the following technical observations on MTC under the event-triggered traffic model:
\begin{enumerate}
    \item The UEs activity is triggered by event concentrated around a very small subset of  \emph{active} clusters, thus, giving rise to an \emph{inner cluster} sparsity structure.
    \item An active cluster refers to any cluster with at least one active UE, while containing at most ${L_\mathrm{c}\leq L}$ active UEs, thus, inducing a correlation between the UEs activity in the form of \emph{intra-cluster} sparsity structure. 
\end{enumerate}  

Therefore, in order to encode the prior knowledge on both the intra and inner-cluster sparsity of the network, we  introduce first  the following parameters:
\begin{enumerate}
    \item The binary indicator vector $\vec{c}=[c_1,\ldots,c_{N_{\mathrm{c}}}]\tran \in \mathbb{B}^{N_{\mathrm{c}}}$,  that controls the intra-cluster sparsity. In particular, we    define $c_l=1$ if the  $l$th cluster is active, and  $c_l=0$ otherwise. Subsequently,  we can statistically model each $c_l$, $l=1,\ldots,N_{\mathrm{c}}$ as a  Bernoulli random variable with $p(c_l=1) =\epsilon$ and $p(c_l=0) = 1-\epsilon$.  Furthermore, since the activity amongst cluster is independent, we express the probability mass function of $\vec{c}$ as
   \begin{equation}\label{eq:Bernouli_c}
 p(\vec{c})=   \prod_{l=1}^{N_\mathrm{c}}\mathcal{B}(\vec{c}_l|\epsilon)    
    \end{equation}
    \item  To enforce the sparsity for the UEs within each active cluster, i.\,e.\ the intra-cluster sparsity, we further  impose a structure on $\vec{R}_i$ as  $\vec{R}=\bar{\gamma}_i\vec{\bar{R}}_i$, where $\vec{\bar{R}}_i$ is a positive definite matrix that captures the spatial correlation
structure in $\vec{x}_i$, and $\bar{\gamma}_i \in \mathbb{R}^+$ is a hyper-parameter that controls the sparsity of the effective channel $\vec{x}_i$.  The main idea here is that when $\bar{\gamma}_i\approx 0$,  the covariance matrix  $\bar{\gamma}_i\vec{R}_i$ would be very small  that we could safely estimate that $\vec{x}_i \sim \mathcal{CN}(\vec{0}, \bar{\gamma}_i\vec{\bar{R}}_i) \approx \vec{0}$, whereas if $\bar{\gamma}>0$, $\vec{x}_i$ would be a non-zero vector. 
%For ease of otaion by defining the set of hyper-paramters $\theta={$ 
   \end{enumerate} 
   Subsequently, using the the structured spike-and-slab prior,  we can model the $i$th effective channel $\vec{x}_i$ belonging to the $l$th cluster as
\begin{equation}\label{spike-slab}
     p(\vec{x}_i|c_l,\vec{R}_i)=(1-c_l)\delta(\vec{x}_i)+c_l \mathcal{CN}(\vec{x}_i;\vec{0},\vec{R}_i).
\end{equation}
Finally, to encode the independence amongst the clusters activity, and the  correlation between  the UEs activity with each cluster, we can model the conditional PDF $p(\vec{X}|\vec{c},\vec{R})$ as 
\begin{equation}\label{eq:P(X)_l}
%\begin{array}{ll}
    %p(\vec{X}|\vec{c},\{\vec{R}\}) &=\prod_{l=1}^C 
    \displaystyle p(\vec{X}|\vec{c},\vec{R})=\prod_{l=1}^{N_\mathrm{c}} p(\vec{X}_{\mathcal{C}_l}|c_l)  =\prod_{l=1}^{N_\mathrm{c}} \bigg[(1-c_l)\delta\big(\vec{X}_{\mathcal{C}_l}\big)+c_l\prod_{i \in {\mathcal{C}_l}} \mathcal{CN}(\vec{x}_i;\vec{0},\vec{R}_i) \bigg], \\
  %   p(c_l)&= \mathcal{B}(c_l|\epsilon)\\
    % p(\gamma_i)=\mathcal{IG}(\gamma_i;a_0,b_0)
%\end{array}
  \end{equation}
where $\delta\big(\vec{X}_{\mathcal{C}_l}\big)=\prod_{i \in {\mathcal{C}_l}}\delta(\vec{x}_i)$.


\end{comment}



\begin{equation}
\begin{array}{ll}\label{eq:map_x_gamma}
\{\hat{\vec{X}},\hat{\gamma},\hat{\Sigmab}\}&\hspace{-3mm}=\underset{\vec{X},\gamma,\Sigmab}{\max}~\displaystyle p(\vec{X},\gamma,\Sigmab|\vec{Y})\\
&\hspace{-3mm}=\underset{\vec{X},\gamma,\Sigmab}{\max}~\displaystyle\frac{p(\gamma,\Sigmab)p(\vec{X}|\gamma,\Sigmab)p(\vec{Y}|\vec{X},\gamma,\Sigmab)}{p(\vec{Y})}\\&\hspace{-3mm}\overset{(a)}{=}\underset{\vec{X},\gamma,\Sigmab}{\max}~\displaystyle{p(\gamma,\Sigmab)p(\vec{X}|\gamma,\Sigmab)p(\vec{Y}|\vec{X})}\\
&\hspace{-3mm}\overset{}{=}\underset{\vec{X},\gamma,\Sigmab}{\min}~\displaystyle{-\log\,p(\vec{Y}|\vec{X})}-\log\,p(\vec{X}|\gamma,\Sigmab)-\log\,p(\gamma,\Sigmab)\\
&\hspace{-3mm}\overset{(b)}{=}\underset{\vec{X},\gamma,\Sigmab}{\min}~\displaystyle\frac{1}{\sigma^2}\|\vec{Y}-\vec{\Phi}\vec{X}\tran\|_{\mathrm{F}}^{2}-\log\,p(\vec{X}|\gamma,\Sigmab)-\log\,p(\Sigmab)-\log\,p(\gamma) \end{array}
\end{equation}
where $(a)$ follows from the Markov chain ${\{\gammab,\vec{\Sigmab}\}\rightarrow\vec{X}\rightarrow\vec{Y}}$ and  because $p(\vec{Y})$ does not affect the maximization and $(b)$ follows from the additive Gaussian noise model in \eqref{eq::Y} and independence of UE activity and channels. 
%and $(b)$ follows from the additive Gaussian noise model in \eqref{eq::Y} and independence of UE activity and channels. 



%In the following, we investigate the 

%a weak sparsity priors imposes a continuous distribution functions with $0$ probability that anthat  drives most of the elemnt , while strong sparsity priors are spike-and-slab distributions.
%Sparsity promoting priors for a variable x ∈ R characterized by continuousdistributions are called weak sparsity priors because they assign zero probabilityto the event that the variable x is exactly zero. This implies that if one wereto draw a finite sample from a weak sparsity prior, one would never observe a sample exactly equal to zero. the Student’s t distribution and the horseshoe prior

